ONCE: Boosting Content-based Recommendation with Both Open- and Closed-source Large Language Models

Personalized content-based recommender systems have become indispensable tools for users to navigate through the vast amount of content available on platforms like daily news websites and book recommendation services. However, existing recommenders face significant challenges in understanding the content of items. Large language models (LLMs), which possess deep semantic comprehension and extensive knowledge from pretraining, have proven to be effective in various natural language processing tasks. In this study, we explore the potential of leveraging both open- and closed-source LLMs to enhance content-based recommendation. With open-source LLMs, we utilize their deep layers as content encoders, enriching the representation of content at the embedding level. For closed-source LLMs, we employ prompting techniques to enrich the training data at the token level. Through comprehensive experiments, we demonstrate the high effectiveness of both types of LLMs and show the synergistic relationship between them. Notably, we observed a significant relative improvement of up to 19.32% compared to existing state-of-the-art recommendation models. These findings highlight the immense potential of both open- and closed-source of LLMs in enhancing content-based recommendation systems. We will make our code and LLM-generated data available for other researchers to reproduce our results.

==> components/cot-k.tex <==
\begin{figure}[b]
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tikzpicture}
\begin{axis}[    
    xlabel={\#generated news articles per new user},
    ylabel={AUC},    
    ymin=60.5,    
    ymax=64.5,    
    ytick={61,62,63,64},
    xtick={1,2,3},    
    xticklabels={0 (MIND), 1, 2 (MIND-UP$\rightarrow$NG)},
    grid=both,    
    legend pos=north west, 
]

    \addplot[c1,mark=*,line width=2pt] coordinates {
        (1, 62.27)
        (2, 63.52)
        (3, 64.02)
    };
    \addlegendentry{PLMNR}
    
    \addplot[c2,mark=square*,line width=2pt] coordinates {
        (1, 61.16)
        (2, 63.11)
        (3, 63.57)
    };
    \addlegendentry{LSTUR}
    
    \addplot[c3,mark=triangle*,line width=2pt] coordinates {
        (1, 61.68)
        (2, 62.95)
        (3, 63.63)
    };
    \addlegendentry{PNN}
    
    \addplot[c4,mark=diamond*,line width=2pt] coordinates {
        (1, 62.00)
        (2, 62.27)
        (3, 63.05)
    };
    \addlegendentry{DCN}

  \end{axis}
\end{tikzpicture}
}
\caption{\label{fig:sm-cot-k}Influence of the number of generated news articles on the chain-based personalized news generator (UP$\rightarrow$NG) over four base models.}
\end{figure}

==> components/cot.tex <==
\begin{table}[b]
\centering
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{2pt}
\caption{\label{tab:sm-cot}Effectiveness of the chain-based personalized news generator ($\text{UP}\rightarrow\text{NG}$). ORI: training with the original data. NG: training with data enhanced by the one-pass personalized news generator.}
\begin{tabular}{ccccccccc}
\toprule
\footnotesize{\textbf{Matching}} & \multicolumn{4}{c}{\textbf{NRMS}} & \multicolumn{4}{c}{\textbf{PLMNR}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} & 61.88 & 30.63 & 31.38 & 37.76 & 62.27 & 31.07 & 31.98 & 38.31 \\
\textbf{NG} & 62.40 & 30.68 & 31.41 & 37.82 & 63.00 & 31.03 & 32.10 & 38.41 \\
\textbf{UP$\rightarrow$NG} & \textbf{62.95} & \textbf{32.00} & \textbf{32.80} & \textbf{39.00} & \textbf{64.02} & \textbf{31.98} & \textbf{33.25} & \textbf{39.40} \\
\midrule
\footnotesize{\textbf{Ranking}} & \multicolumn{4}{c}{\textbf{PNN}} & \multicolumn{4}{c}{\textbf{DIN}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} & 61.68 & 29.21 & 29.72 & 36.44 & 60.80 & 28.45 & 28.87 & 35.60 \\
\textbf{NG} & 62.25 & 29.51 & 30.12 & 36.87 & 62.87 & 30.42 & 30.88 & 37.70 \\
\textbf{UP$\rightarrow$NG} & \textbf{63.63} & \textbf{30.85} & \textbf{31.14} & \textbf{38.69} & \textbf{63.53} & \textbf{30.76} & \textbf{31.21} & \textbf{38.13} \\
\bottomrule
\end{tabular}
\end{table}

==> figures-v2/content_rs.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{images-v2/ContentRS.pdf}
    \caption{\label{fig:content_rs} General content-based recommendation model.}
\end{figure}


==> figures-v2/open-source.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=.7\linewidth]{images-v2/Open-Source.pdf}
    \caption{\label{fig:open_source} Tuning open-source LLMs as content encoder.}
\end{figure}


==> figures/chat.tex <==
\begin{figure*}[!ht]
    \centering
    % \setlength\tabcolsep{2pt}
    \resizebox{0.90\linewidth}{!}{
    \begin{tabular}{ccc}
    \begin{subfigure}{0.3\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/Chat-FE}
        }
        \caption{\label{fig:chat-fe} Given: news title, abstract, and category. Response: enhanced news title.}
    \end{subfigure} &
    \begin{subfigure}{0.3\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/Chat-UM}
        }
        \caption{\label{fig:chat-um}Given: title of news list read by user. \\ Response: user interests.}
    \end{subfigure} &
    \begin{subfigure}{0.3\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/Chat-IG}
        }
        \caption{\label{fig:chat-ig}Given: title and category of news list read by user. Response: generated news.}
    \end{subfigure} \\
    \end{tabular}
    }

    \caption{\label{fig:chat} Illustration of three perspectives of LLM-based data augmentation. Texts with gray background are sent by us, and that with green background are responded by ChatGPT. Texts with tag icon, in bold, and in light gray are news category, title, and abstract, respectively. We simplify the prompt for the demonstration purpose. The complete prompt is available in the Method section, and the response from ChatGPT can be found at our publicly accessible link.}
\end{figure*}


==> figures/idea.tex <==
\begin{figure*}[t]
    \centering
    \includegraphics[width=\linewidth]{images/Framework.pdf}
    \caption{\label{fig:idea} 
    %An overview of LLM-powered GENRE (generative news recommendation) framework.
    Our proposed LLM-powered generative news recommendation (GENRE) framework.
    }
\end{figure*}

==> figures/newsencoder.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.95\linewidth]{images/NewsEncoder3}
    \caption{\label{fig:newsencoder} General multi-modal news encoder.}
\end{figure}

==> figures/overview.tex <==
\begin{figure*}[t]
    \centering
    \setlength\tabcolsep{15pt}
    \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{cc}
    \begin{subfigure}{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/NRS-OR2}
        }
        \caption{\label{fig:ov-or}General news recommender}
    \end{subfigure} &
    \begin{subfigure}{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/NRS-FE2}
        }
        \caption{\label{fig:ov-fe}News recommender with LLM-enhanced news titles}
    \end{subfigure} \\
    \begin{subfigure}{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/NRS-UM2}
        }
        \caption{\label{fig:ov-um}News recommender with LLM-generated user profiles}
    \end{subfigure} &
    \begin{subfigure}{0.5\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/NRS-IG2}
        }
        \caption{\label{fig:ov-ig}News recommender with LLM-generated personalized news pieces}
    \end{subfigure} \\
    \end{tabular}
    }

    \caption{\label{fig:overview} %Overview of the integration of the LLM-empowered generated data from three GENRE instances into the news recommendation models. We only provide a high-level integration pipeline, ignoring the implementation details of the recommendation models. The interaction module is involved in the prediction.
    Illustration of the downstream training of news recommenders in different scenarios.
    }
\end{figure*}

==> figures/prompt-cot.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=\linewidth]{images/CoT2.pdf}
    \caption{\label{fig:prompt-cot} Chain-based personalized news generator.}
\end{figure}

==> figures/prompt-fe.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=0.65\linewidth]{images/PC-FE.pdf}
    \caption{\label{fig:prompt-fe} Prompt designed for news feature enhancer.}
\end{figure}

==> figures/prompt-ig.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.65\linewidth]{images/PC-IG.pdf}
    \caption{\label{fig:prompt-ig} Prompt designed for user interest generator.}
\end{figure}

==> figures/prompt-um.tex <==
\begin{figure}[h]
    \centering
    \includegraphics[width=0.65\linewidth]{images/PC-UM.pdf}
    \caption{\label{fig:prompt-um} Prompt designed for user profile modeler.}
\end{figure}

==> figures/prompt.tex <==
\begin{figure*}[t]
    \centering
    % \setlength\tabcolsep{20pt}
    % \resizebox{1.0\linewidth}{!}{
    \begin{tabular}{ccc}
    \begin{subfigure}{0.33\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/PC-FE}
        }
        \caption{\label{fig:pt-fe}News summarizer}
    \end{subfigure} &
    \begin{subfigure}{0.33\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/PC-UM}
        }
        \caption{\label{fig:pt-um}User profiler}
    \end{subfigure} &
    \begin{subfigure}{0.33\textwidth}
        \resizebox{1.0\linewidth}{!}{
            \includegraphics{images/PC-IG}
        }
        \caption{\label{fig:pt-ig}Personalized news generator}
    \end{subfigure} \\
    \end{tabular}
    % }

    \caption{\label{fig:prompt} %Prompt designed from three perspectives.
     Prompts designed under our GENRE framework.}
\end{figure*}

==> tables/big-fe.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{3pt}
\caption{\label{tab:big-fe}Effectiveness of the news summarizer ($\text{NS}$). $\text{ORI}$: training with the original data.}
\begin{tabular}{ccccccccc}
\toprule[1pt]
\footnotesize{\textbf{Matching}} & \multicolumn{2}{c}{\textbf{NAML}} & \multicolumn{2}{c}{\textbf{LSTUR}} & \multicolumn{2}{c}{\textbf{NRMS}} & \multicolumn{2}{c}{\textbf{PLMNR}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} \\
\midrule
\textbf{AUC} & 61.75 & \textbf{63.73} & 61.27 & \textbf{62.16} & 61.71 & \textbf{63.85} & 62.53 & \textbf{64.80} \\
\textbf{MRR} & 30.60 & \textbf{31.83} & 29.64 & \textbf{30.52} & 30.20 & \textbf{31.57} & 30.74 & \textbf{33.08} \\
\textbf{N@5} & 31.35 & \textbf{32.94} & 30.28 & \textbf{31.27} & 30.98 & \textbf{32.35} & 31.31 & \textbf{34.25} \\
\textbf{N@10} & 37.85 & \textbf{39.24} & 36.76 & \textbf{37.85} & 37.42 & \textbf{38.80} & 38.03 & \textbf{40.35} \\
\midrule[1pt]
\footnotesize{\textbf{Ranking}} & \multicolumn{2}{c}{\textbf{BST}} & \multicolumn{2}{c}{\textbf{DCN}} & \multicolumn{2}{c}{\textbf{PNN}} & \multicolumn{2}{c}{\textbf{DIN}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} & \textbf{ORI} & \textbf{NS} \\
\midrule
\textbf{AUC} & 61.73 & \textbf{62.85} & 62.63 & \textbf{64.19} & 61.75 & \textbf{63.85} & 60.95 & \textbf{61.26} \\
\textbf{MRR} & 29.84 & \textbf{31.51} & 29.73 & \textbf{31.96} & 29.45 & \textbf{31.54} & 28.13 & \textbf{29.72} \\
\textbf{N@5} & 30.55 & \textbf{32.16} & 30.52 & \textbf{32.67} & 29.99 & \textbf{32.38} & 28.77 & \textbf{30.38} \\
\textbf{N@10} & 37.22 & \textbf{38.78} & 37.12 & \textbf{39.16} & 36.67 & \textbf{38.78} & 35.42 & \textbf{36.76} \\
\bottomrule[1pt]
\end{tabular}
\end{table}

==> tables/big-ig.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{3pt}
\caption{\label{tab:big-ig}Effectiveness of the personalized news generator ($\text{NG}$). $\text{ORI}$: training with the original data.}
\begin{tabular}{ccccccccc}
\toprule[1pt]
\footnotesize{\textbf{Matching}} & \multicolumn{2}{c}{\textbf{NAML}} & \multicolumn{2}{c}{\textbf{LSTUR}} & \multicolumn{2}{c}{\textbf{NRMS}} & \multicolumn{2}{c}{\textbf{PLMNR}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} \\
\midrule
\textbf{AUC} & 61.75 & \textbf{62.93} & 61.27 & \textbf{63.88} & 61.71 & \textbf{63.04} & 62.53 & \textbf{63.11} \\
\textbf{MRR} & 30.60 & \textbf{30.83} & 29.64 & \textbf{31.76} & 30.20 & \textbf{31.00} & 30.74 & \textbf{30.90} \\
\textbf{N@5} & 31.35 & \textbf{32.10} & 30.28 & \textbf{32.92} & 30.98 & \textbf{31.84} & 31.31 & \textbf{32.02} \\
\textbf{N@10} & 37.85 & \textbf{38.34} & 36.76 & \textbf{39.16} & 37.42 & \textbf{38.22} & 38.03 & \textbf{38.37} \\
\midrule[1pt]
\footnotesize{\textbf{Ranking}} & \multicolumn{2}{c}{\textbf{BST}} & \multicolumn{2}{c}{\textbf{DCN}} & \multicolumn{2}{c}{\textbf{PNN}} & \multicolumn{2}{c}{\textbf{DIN}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} & \textbf{ORI} & \textbf{NG} \\
\midrule
\textbf{AUC} & 61.73 & \textbf{62.86} & 62.63 & \textbf{62.67} & 61.75 & \textbf{62.24} & 60.95 & \textbf{62.18} \\
\textbf{MRR} & 29.84 & \textbf{30.54} & 29.73 & \textbf{29.81} & 29.45 & \textbf{29.34} & 28.13 & \textbf{29.33} \\
\textbf{N@5} & 30.55 & \textbf{31.32} & 30.52 & \textbf{30.63} & 29.99 & \textbf{30.05} & 28.77 & \textbf{29.88} \\
\textbf{N@10} & 37.22 & \textbf{37.93} & 37.12 & \textbf{37.18} & 36.67 & \textbf{36.73} & 35.42 & \textbf{36.79} \\
\bottomrule[1pt]
\end{tabular}
\end{table}

==> tables/big-pm.tex <==
\begin{table}[]
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{3pt}
\caption{\label{tab:big-pm}Effectiveness of the user profiler ($\text{UP}$). $\text{ORI}$: training with the original data.}
\begin{tabular}{ccccccccc}
\toprule[1pt]
\footnotesize{\textbf{Matching}} & \multicolumn{2}{c}{\textbf{NAML}} & \multicolumn{2}{c}{\textbf{LSTUR}} & \multicolumn{2}{c}{\textbf{NRMS}} & \multicolumn{2}{c}{\textbf{PLMNR}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
 & \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} \\
\midrule
\textbf{AUC} & 61.75 & \textbf{62.19} & 61.27 & \textbf{61.81} & 61.71 & \textbf{61.90} & 62.53 & \textbf{63.31} \\
\textbf{MRR} & 30.60 & \textbf{30.90} & 29.64 & \textbf{30.39} & 30.20 & \textbf{30.60} & 30.74 & \textbf{31.58} \\
\textbf{N@5} & 31.35 & \textbf{31.78} & 30.28 & \textbf{31.00} & 30.98 & \textbf{31.54} & 31.31 & \textbf{32.65} \\
\textbf{N@10} & 37.85 & \textbf{38.26} & 36.76 & \textbf{37.46} & 37.42 & \textbf{37.66} & 38.03 & \textbf{38.87} \\
\midrule[1pt]
\footnotesize{\textbf{Ranking}} & \multicolumn{2}{c}{\textbf{BST}} & \multicolumn{2}{c}{\textbf{DCN}} & \multicolumn{2}{c}{\textbf{PNN}} & \multicolumn{2}{c}{\textbf{DIN}} \\
\cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9}
& \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} & \textbf{ORI} & \textbf{UP} \\
\midrule
\textbf{AUC} & 61.73 & \textbf{62.67} & 62.63 & \textbf{63.47} & 61.75 & \textbf{62.34} & 60.95 & \textbf{62.65} \\
\textbf{MRR} & 29.84 & \textbf{30.75} & 29.73 & \textbf{29.92} & 29.45 & \textbf{29.67} & 28.13 & \textbf{30.74} \\
\textbf{N@5} & 30.55 & \textbf{31.63} & 30.52 & \textbf{30.66} & 29.99 & \textbf{30.46} & 28.77 & \textbf{31.50} \\
\textbf{N@10} & 37.22 & \textbf{38.01} & 37.12 & \textbf{37.47} & 36.67 & \textbf{37.07} & 35.42 & \textbf{38.05} \\
\bottomrule[1pt]
\end{tabular}
\end{table}

==> tables/big-table.tex <==
\begin{table*}[t]
\renewcommand{\arraystretch}{1.3} 
\setlength\tabcolsep{4pt}
\caption{\label{tab:big-table}Comparison of GENRE-based augmented data with original data among different base models. We use $ORI$, $FE$, $PT$, and $IG$ to represent the original data, data augmented by feature enhancer, user modeler, and interest generator, respectively. We bold the best result in each row.}
\resizebox{\linewidth}{!}{
\begin{tabular}{ccccccccccccccccccccc}
\toprule[1pt]
& \multicolumn{4}{c}{\textbf{NAML}} & \multicolumn{4}{c}{\textbf{LSTUR}} & \multicolumn{4}{c}{\textbf{NRMS}} & \multicolumn{4}{c}{\textbf{PLMNR}}  & \multicolumn{4}{c}{\textbf{MINER}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
& \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} 
    & 61.75 & 30.60 & 31.35 & 37.85 
    & 61.27 & 29.64 & 30.28 & 36.76 
    & 61.71 & 30.20 & 30.98 & 37.42 
    & 62.53 & 30.74 & 31.31 & 38.03 \\
\textbf{FE} 
    & \textbf{63.73} & \textbf{31.83} & \textbf{32.94} & \textbf{39.24} 
    & 62.16 & 30.52 & 31.27 & 37.85 
    & \textbf{63.85} & \textbf{31.57} & \textbf{32.35} & \textbf{38.80} 
    & \textbf{64.80} & \textbf{33.08} & \textbf{34.25} & \textbf{40.35} \\
\textbf{PT} 
    % & 63.23 & 31.69 & 32.60 & 39.04 
    % & 64.74 & 32.22 & 33.54 & 39.71 
    % & 63.55 & 32.20 & 33.60 & 39.51 
    % & 64.17 & 31.95 & 33.08 & 39.40 \\
    & 62.19 & 30.90 & 31.78 & 38.26 
    & 61.81 & 30.39 & 31.00 & 37.46 
    & 61.90 & 30.60 & 31.54 & 37.66 
    & 63.31 & 31.58 & 32.65 & 38.87 \\
\textbf{IG} 
    & 62.93 & 30.83 & 32.10 & 38.34 
    & \textbf{63.88} & \textbf{31.76} & \textbf{32.92} & \textbf{39.16} 
    & 63.04 & 31.00 & 31.84 & 38.22 
    & 63.11 & 30.90 & 32.02 & 38.37 \\
    % & 62.38 & 30.79 & 31.90 & 38.13
    % & 62.29 & 30.68 & 31.54 & 38.02 
    % & 61.87 & 30.42 & 31.14 & 37.50 
    % & 62.73 & 30.90 & 31.89 & 38.33 \\
% \textbf{ALL}
%     &  &  &  &  
%     &  &  &  &  
%     &  &  &  &  
%     &  &  &  &  \\
\midrule[1pt]
& \multicolumn{4}{c}{\textbf{BST}} & \multicolumn{4}{c}{\textbf{DCN}} & \multicolumn{4}{c}{\textbf{PNN}} & \multicolumn{4}{c}{\textbf{DIN}} & \multicolumn{4}{c}{\textbf{Fastformer}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9} \cmidrule(lr){10-13} \cmidrule(lr){14-17} \cmidrule(lr){18-21}
& \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} 
    & 61.73 & 29.84 & 30.55 & 37.22
    & 62.63 & 29.73 & 30.52 & 37.12 
    & 61.75 & 29.45 & 29.99 & 36.67 
    & 60.95 & 28.13 & 28.77 & 35.42 \\
\textbf{FE} 
    & 62.85 & \textbf{31.51} & \textbf{32.16} & \textbf{38.78} 
    & \textbf{64.19} & \textbf{31.96} & \textbf{32.67} & \textbf{39.16} 
    & \textbf{63.85} & \textbf{31.54} & \textbf{32.38} & \textbf{38.78}
    & 61.26 & 29.72 & 30.38 & 36.76 \\
\textbf{PT} 
    & 62.67 & 30.75 & 31.63 & 38.01
    & 63.47 & 29.92 & 30.66 & 37.47 
    & 62.34 & 29.67 & 30.46 & 37.07 
    & \textbf{62.65} & \textbf{30.74} & \textbf{31.50} & \textbf{38.05} \\
\textbf{IG} 
    % & 63.71 & 31.05 & 32.01 & 38.41 
    % & 62.67 & 29.81 & 30.63 & 37.18 
    % & 62.02 & 29.40 & 30.01 & 36.76 
    % & 61.32 & 28.36 & 28.71 & 35.67  \\
    & \textbf{62.86} & 30.54 & 31.32 & 37.93 
    & 62.67 & 29.81 & 30.63 & 37.18 
    & 62.24 & 29.34 & 30.05 & 36.73 
    & 62.18 & 29.33 & 29.88 & 36.79  \\
% \textbf{ALL}
%     &  &  &  &  
%     &  &  &  &  
%     &  &  &  &  
%     &  &  &  &  \\
\bottomrule[1pt]
\end{tabular}
}
\end{table*}


==> tables/cot.tex <==
% \begin{table}[t]
% \centering
% \renewcommand{\arraystretch}{1.3} 
% \setlength\tabcolsep{2pt}
% \caption{\label{tab:cot}Effectiveness comparison among ORIginal dataset $\text{ORI}$, one-pass personalized news generation $\text{NG}$, and chain-based personalized news generation $\text{UP}\rightarrow\text{NG}$.}
% \begin{tabular}{ccccccccc}
% \toprule
%  & \multicolumn{4}{c}{\textbf{NAML}} & \multicolumn{4}{c}{\textbf{LSTUR}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
%  & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
% \midrule
% \textbf{ORI} & 59.29 & 28.46 & 29.34 & 35.64 & 56.64 & 26.63 & 26.81 & 33.26 \\
% \textbf{NG} & 59.71 & 28.74 & 29.46 & 35.82 & 57.80 & 27.20 & 27.79 & 33.86 \\
% \textbf{UP$\rightarrow$NG} & \textbf{60.69} & \textbf{29.06} & \textbf{29.93} & \textbf{36.26} & \textbf{58.48} & \textbf{27.85} & \textbf{28.47} & \textbf{34.69} \\
% \midrule
%  & \multicolumn{4}{c}{\textbf{BST}} & \multicolumn{4}{c}{\textbf{DCN}} \\
% \cmidrule(lr){2-5} \cmidrule(lr){6-9}
% \textbf{} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
% \midrule
% \textbf{ORI} & 60.03 & 29.09 & 29.69 & 36.17 & 59.01 & 27.20 & 27.11 & 34.18 \\
% \textbf{NG} & 60.42 & 29.43 & 30.10 & 36.47 & 61.05 & 28.93 & 29.13 & 36.41 \\
% \textbf{UP$\rightarrow$NG} & \textbf{61.13} & \textbf{30.25} & \textbf{31.01} & \textbf{37.28} & \textbf{62.27} & \textbf{29.74} & \textbf{30.23} & \textbf{37.13} \\
% \bottomrule
% \end{tabular}
% \end{table}


\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{2pt}
\caption{\label{tab:cot}Effectiveness of the chain-based personalized news generator ($\text{UP}\rightarrow\text{NG}$). ORI: training with the original data. NG: training with data enhanced by the one-pass personalized news generator.}
\begin{tabular}{ccccccccc}
\toprule
\footnotesize{\textbf{Matching}} & \multicolumn{4}{c}{\textbf{NAML}} & \multicolumn{4}{c}{\textbf{LSTUR}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
 & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} & 61.17 & 29.71 & 30.32 & 36.99 & 61.16 & 29.58 & 30.17 & 36.69 \\
\textbf{NG} & 62.57 & 30.94 & 32.27 & 38.35 & 62.70 & 30.87 & 31.72 & 38.18 \\
\textbf{UP$\rightarrow$NG} & \textbf{63.61} & \textbf{31.58} & \textbf{32.63} & \textbf{39.07} & \textbf{63.57} & \textbf{31.43} & \textbf{32.62} & \textbf{39.01} \\
\midrule
\footnotesize{\textbf{Ranking}} & \multicolumn{4}{c}{\textbf{BST}} & \multicolumn{4}{c}{\textbf{DCN}} \\
\cmidrule(lr){2-5} \cmidrule(lr){6-9}
& \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} & \textbf{AUC} & \textbf{MRR} & \textbf{N@5} & \textbf{N@10} \\
\midrule
\textbf{ORI} & 61.20 & 29.34 & 29.78 & 36.54 & 62.00 & 29.36 & 30.22 & 36.74 \\
\textbf{NG} & 62.45 & 30.20 & 31.03 & 37.49 & 62.65 & \textbf{29.87} & \textbf{30.74} & \textbf{37.23} \\
\textbf{UP$\rightarrow$NG} & \textbf{63.28} & \textbf{31.49} & \textbf{32.45} & \textbf{38.84} & \textbf{63.05} & 29.79 & 30.61 & \textbf{37.23} \\
\bottomrule
\end{tabular}
\end{table}


==> tables/models.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{1.2} 
\setlength\tabcolsep{0pt}
\centering
\caption{\label{tab:models} Architectures of the recommendation models. Top: matching-based models. Bottom: ranking-based models.}
\resizebox{1.0\linewidth}{!}{
\begin{tabular}{cccc}
\toprule
\textbf{Model} & \textbf{News Encoder} & \textbf{User Encoder} & \textbf{Interaction Module} \\
\midrule
\textbf{NAML~\cite{naml}} & CNN~\cite{cnn} & Attention~\cite{ada} & Dot Product \\
\textbf{LSTUR~\cite{lstur}} & CNN~\cite{cnn} & GRU~\cite{gru} & Dot Product \\
\textbf{NRMS~\cite{nrms}} & Attention~\cite{attention} & Attention~\cite{attention} & Dot Product \\
\textbf{PLMNR~\cite{plmnr}} & Attention~\cite{attention} & Transformer~\cite{attention} & Dot Product \\
\midrule
\textbf{BST~\cite{bst}} & Pooling & Transformer~\cite{attention} & MLP \\
\textbf{DCN~\cite{dcn}} & Pooling & Pooling & Deep \& Cross \\
\textbf{PNN~\cite{pnn}} & Pooling & Pooling & Inner Product \\
\textbf{DIN~\cite{din}} & Pooling & N/A & Attention~\cite{din} \\
\bottomrule
\end{tabular}
}
\end{table}

